Optimizing Polynomial Multiplication and Fixed-Weight Sampling for HQC on ARM Cortex-M4

In this paper, we present an optimized implementation of Hamming Quasi-Cyclic (HQC) on the ARM Cortex-M4. We optimize (i) the polynomial multiplication and (ii) the support expansion in fixed-weight sampling, and (iii) propose an optional caching strategy that reuses the public transforms and hash recomputed under a fixed key. For the polynomial multiplication, the fixed-constant multiplications in the Frobenius additive FFT (FAFFT) butterfly spend nearly half of their instructions on VMOV data movements between general-purpose and floating-point registers rather than arithmetic. Because minimizing the XOR count alone can increase the total instruction count, we propose a dirty-aware register-allocation policy and an XOR-operation reordering that reduce the VMOV count by up to 48.1% while leaving the XOR count unchanged. We apply these to a multiplication that combines prior FAFFT-CRT methods, and for HQC-1 we further find a 34% sparser FAFFT modulus that lowers the CRT reconstruction cost. For fixed-weight sampling, we rewrite the support expansion with predicated execution and 4-way unrolling, lowering the per-word cost of its inner loop from 22 to 6 cycles while remaining constant-time. On the NUCLEO-L4R5ZI board, our implementation reduces key generation, encapsulation, and decapsulation by up to 33.1%, 34.6%, and 29.8% over the faster of the two prior state-of-the-art implementations, and the optional caching yields a further reduction of up to 32.7% and 18.9% for encapsulation and decapsulation.

==> settings.tches.tex <==
\setfirstpage{0}
\setlastpage{0}
\setvolume{0}
\setnumber{0}

\setISSN{2569-2925}
\makeatletter
\setDOI{10.46586/tches.v\IACR@vol.i\IACR@no.\IACR@fp-\IACR@lp}
\makeatother

\setkeys{IACR}{journal=tches}

